$Z^*$: Zero-shot Style Transfer via Attention Rearrangement

Despite the remarkable progress in image style transfer, formulating style in the context of art is inherently subjective and challenging. In contrast to existing learning/tuning methods, this study shows that vanilla diffusion models can directly extract style information and seamlessly integrate the generative prior into the content image without retraining. Specifically, we adopt dual denoising paths to represent content/style references in latent space and then guide the content image denoising process with style latent codes. We further reveal that the cross-attention mechanism in latent diffusion models tends to blend the content and style images, resulting in stylized outputs that deviate from the original content image. To overcome this limitation, we introduce a cross-attention rearrangement strategy. Through theoretical analysis and experiments, we demonstrate the effectiveness and superiority of the diffusion-based $\underline{Z}$ero-shot $\underline{S}$tyle $\underline{T}$ransfer via $\underline{A}$ttention $\underline{R}$earrangement, Z-STAR.

==> Figs/fig_compare_test.tex <==
\begin{figure*}%[h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{image/compare.pdf}
\vspace{-15pt}
\caption{Qualitative comparisons of style transfer results using different methods.}
\label{fig:compare}
\vspace{-3pt}
\end{figure*}


==> Figs/fig_content_leak.tex <==
\newcommand\biascomparisonfigurewidth{0.075}
\newcommand\biascomparisontextwidth{0.015}

\begin{figure*}
\centering
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/StyleFormer-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/iest-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mast-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/sanet-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/avatar-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/s1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/StyleFormer-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/iest-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mast-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/sanet-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/avatar-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp1-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

% \begin{minipage}{\biascomparisontextwidth\linewidth}
%     \centering
%     \rotatebox{90}{\figtext{Style}}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/s5.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc5-20.png}
% \end{minipage}
% % \begin{minipage}{\biascomparisonfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% % \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisontextwidth\linewidth}
%     \centering
%     \rotatebox{90}{\figtext{Round 20}}
% \end{minipage}
\vspace{1pt}

\hspace{0.07\linewidth}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{StyleFormer}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{IEST}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{ArtFlow}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{MAST}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{SANet}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{Avatar}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Visualization of the content leak issue. Top/bottom: results after running the same stylization process using a certain method after the \engordnumber{1} and the \engordnumber{20} round, respectively.}
\vspace{-5pt}
\label{fig:content_leak}
\end{figure*}


==> Figs/fig_content_leak_s.tex <==
\newcommand\biascomparisonfigurewidth{0.13}
\newcommand\biascomparisontextwidth{0.015}

\begin{figure*}
\centering
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c2.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth,height=\linewidth]{image/figs_bias_comparison/s2.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc2-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp1-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c3.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc3-1.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-1.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth,height=\linewidth]{image/figs_bias_comparison/s3.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc3-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c4.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc4-1.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-1.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth,height=\linewidth]{image/figs_bias_comparison/s4.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc4-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c5.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc5-1.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-1.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/s5.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc5-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\hspace{0.13\linewidth}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{ArtFlow}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}
%\includegraphics[width= 0.99 \linewidth]{image/content_leak.pdf}
\vspace{-5pt}
\caption{Visualizations of the content leak issue.}
\vspace{-5pt}
\label{fig:content_leak_s}
\end{figure*}


==> Figs/fig_diff.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/diff_compare.pdf}
\caption{
% Compared with close-domain diffusion-based style transfer method. The effectiveness of StyleDiff is constrained when confronted with images that deviate from the specific training domain. This limitation is evident in the perplexing outcomes depicted in the first two columns of the third row.
Differentiating itself from diffusion-based style transfer methods tailored for specific domains, StyleDiff demonstrates limitations in effectively handling images that deviate from the training domain. This constraint becomes evident when scrutinizing the perplexing outcomes presented in the first two columns of the third row. Nevertheless, our proposed method exhibits consistent and satisfactory performance across all types of input images.
}
% \vspace{-4mm}
\label{fig:diff}
\vspace{-10pt}
\end{figure}

==> Figs/fig_inst.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/inst_compare.pdf}
\caption{Compared with open-domain diffuison-based style transfer methods. Inst damage the content structure Seriously. The style in the results of VCT deviate from the references. }
% \vspace{-4mm}
\label{fig:inst}
\vspace{-10pt}
\end{figure}

==> Figs/fig_limitation.tex <==
\begin{figure}[h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{image/bad_case.pdf}
\caption{Limitation of our StyTr$^2$ framework.
}
\label{fig:bad_case}
\end{figure}

==> Figs/fig_pe_visualization.tex <==
% \begin{figure}%[t]
%     \setlength{\abovecaptionskip}{2mm}
%     \centering
%     \includegraphics[width=\linewidth]{image/stytr2_cape_visual.pdf}
%     \vspace{-12pt}
%     \caption{Normalized attention scores of different types of PE.}
%     \label{fig:stytr2_cape_visual}
% \end{figure}

\begin{figure}
    \setlength{\abovecaptionskip}{2mm}
    \centering
    \begin{minipage}{\linewidth}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/Learnable_PE.png}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/Sinusoidal_PE.png}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/CAPE1.png}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/CAPE2.png}
    \end{minipage}
    \vspace{-1pt}
    \begin{minipage}{0.24\linewidth}
        \centering
        \figtext{Learnable PE}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \figtext{Sinusoidal PE}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \centering
        \figtext{CAPE}
    \end{minipage}

    \caption{Normalized attention scores of different types of PE.}
    \label{fig:stytr2_cape_visual}
\end{figure}


==> Figs/fig_style_gradient.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/diff_style_gradient.pdf}
\caption{An illustration of horizontal styling gradient created by our method.}
% \vspace{-4mm}
\label{fig:style_grad}
\vspace{-10pt}
\end{figure}

==> Figs/fig_sup1.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/experiment1.pdf}
\caption{Compared with other style transfer methods. The content images are presented in first column, the style images are presented in second column, and the stylized results generated by different methods are presented in the rest. 
}
% \vspace{-2mm}
\label{fig:sup1}
%\vspace{-10pt}
\end{figure*}

==> Figs/fig_sup2.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/experiment2.pdf}
\caption{Compared with other style transfer methods. The content images are presented in first column, the style images are presented in second column, and the stylized results generated by different methods are presented in the rest. 
}
% \vspace{-2mm}
\label{fig:sup2}
%\vspace{-10pt}
\end{figure*}

==> Figs/fig_sup3.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow7.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc7.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain7.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow8.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}


\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc8.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain8.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow9.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc9.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain9.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup3}
\end{figure*}


==> Figs/fig_sup4.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow10.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc10.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain10.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow11.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc11.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain11.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow12.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc12.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain12.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup4}
\end{figure*}

==> Figs/fig_supp_ItoS.tex <==
% \begin{figure}%[!ht]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width= \linewidth]{image/ItoS2.pdf}
% \caption{Comparisons of CNN and Linear projection through several rounds of image stylization.
% }
% \label{fig:ItoS2}
% \end{figure}

\newcommand\Ttosfigurewidth{0.22}
\newcommand\Ttostextwidth{0.015}
% \newcommand\nTtostextwidth{0.007}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/s.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l1.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l2.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l3.png}
\end{minipage}
\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Linear}}
\end{minipage}

\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/c.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn1.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn2.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn3.png}
\end{minipage}
\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{CNN}}
\end{minipage}

\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Input}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 1}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 2}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 3}
\end{minipage}
\caption{Comparisons of CNN based and our linear projection based layers through several rounds of image stylization.
}
\vspace{-2mm}
\label{fig:ItoS2}
\end{figure}

==> Figs/fig_supp_big.tex <==
\newcommand\bigfigurewidth{0.31}

\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c1.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r1.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s1.png}


\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c2.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r2.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s2.png}

\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c3.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r3.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s3.png}

\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c4.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r4.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s4.png}

\vspace{-2pt}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Our results}
\end{minipage}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\vspace{-7pt}
\caption{More style transfer results in a large resolution of $768 \times 768$.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}\label{fig:big}
\end{figure*}


==> Figs/fig_supp_noise.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\textwidth]{image/noise}
\caption{Comparisons of model robustness with ArtFlow. We visualize the impact of adding a small perturbation $\Delta$ following a Gaussian distribution on the stylized images in the \engordnumber{4} and \engordnumber{7} columns.
}
\label{fig:noise}
\end{figure*}


==> Figs/fig_supp_progressive.tex <==
\newcommand\pecomparisonfigurewidth{0.24}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/pure_position.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/c.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/single.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/m.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/s.PNG}
% \includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}

\vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Single-layer}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Multi-layer}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\caption{Impact of progressive generation of transformer decoder.}
\label{fig:progressive}
\end{figure}


==> Figs/fig_supp_weights.tex <==
% \begin{figure}%[!h]
% \setlength{\abovecaptionskip}{0mm}
% \centering
% \includegraphics[width= \linewidth]{image/weight.pdf}
% \caption{Impact of style weight.
% }
% \label{fig:weight}
% \end{figure}

\newcommand\weightfigurewidth{0.24}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/pure_position.pdf}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/c1.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wl1.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wh1.png}
\includegraphics[width=\weightfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_weight/s1.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}

\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/c2.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wl2.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wh2.png}
\includegraphics[width=\weightfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_weight/s2.png}

\vspace{-4pt}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{$\lambda_{s} = 5$}
\end{minipage}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{$\lambda_{s} = 10$}
\end{minipage}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\caption{Impact of style weight.}
\vspace{-2mm}
\label{fig:weight}
\end{figure}


==> Figs/fig_teaser.tex <==
%\begin{figure*}[t]
%\setlength{\abovecaptionskip}{2mm}
%\centering
%\includegraphics[width=\linewidth]{image/intermediate_layers.pdf}
%\caption{
%Comparisons of intermediate layers using the rightmost image as both the content and the style image in a reconstruction task.
% (a) Our method. We decode the features extracted in the first three layers of our transformer decoder.
% The reconstruction results maintain distinct structures with increasing detailed brushstrokes.
% Since transformer can obtain long-range dependencies, the results generated by each layer look visually promising.
% (b) The CNN-based method proposed by Gatys et al.~\cite{gatys:2016:image}. We reconstruct the input image from from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network.
%(a) Image reconstruction results from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network based on Gatys et al.~\cite{gatys:2016:image}.
%(b) Feature visualizations of three layers of the transformer decoder.
% We find that reconstruction results match the style of a given image on an increasing scale as the network deepens.
% Different layers of CNN-based model focus on different scale information, thus it cannot generate satisfactory result by every layer.
%}
%\label{fig:pipline}
%\end{figure*}


\begin{center}
    \centering
    \captionsetup{type=figure}
\includegraphics[width=0.8 \linewidth]{image/teaser.pdf}
\caption{
Our stylization results. Our method can generate promising stylized effect with well-preserved content structures and fine details.
}
\label{fig:teaser}
\end{center}

==> Figs/fig_user_study.tex <==
\begin{table*}%[!h]
\small
% \setlength\tabcolsep{9.5pt}
\centering
\begin{floatrow}

\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\end{floatrow}
\vspace{-4mm}
\end{table*}

==> Figs/fig_vis.tex <==
\newcommand\teaserfigurewidth{0.23}
\newcommand\teasertextvspace{-2pt}

\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/intermediate_layers.pdf}
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/input.png}
\end{minipage}
\vspace{\teasertextvspace}
%\begin{minipage}[t]{\linewidth}
\centering
\smallfigtext{\emph{Woman with a Hat}, Henri Matisse, 1905.}
%\end{minipage}
\end{minipage}
% 1st
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/cnn1.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{conv1\_1}
\end{minipage}

\vspace{7pt}
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/ours1.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{layer\_1}
\end{minipage}
%
\end{minipage}
% 2nd
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/cnn2.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{\{conv1\_1,conv2\_1\}}
\end{minipage}

\vspace{7pt}
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/ours2.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{layer\_2}
\end{minipage}
%
\end{minipage}
% 3nd
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/cnn3.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{\{conv1\_1,...,conv4\_1\}}
\end{minipage}

\vspace{7pt}
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/ours3.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{layer\_3}
\end{minipage}
%
\end{minipage}
% text
\begin{minipage}{0.03\linewidth}
    \centering
    \figtext{(a)}

    \vspace{55pt}

    \figtext{(b)}
\end{minipage}
\caption{Comparisons of intermediate layers using the leftmost image as the input content and the style reference in a style transfer task.
% (a) Our method. We decode the features extracted in the first three layers of our transformer decoder.
% The reconstruction results maintain distinct structures with increasing detailed brushstrokes.
% Since transformer can obtain long-range dependencies, the results generated by each layer look visually promising.
% (b) The CNN-based method proposed by Gatys et al.~\cite{gatys:2016:image}. We reconstruct the input image from from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network.
(a) Feature visualizations of a pretrained VGG based on Gatys \etal~\cite{gatys:2016:image}.
(b) Feature visualizations of our transformer decoder.
% We find that reconstruction results match the style of a given image on an increasing scale as the network deepens.
% Different layers of CNN-based model focus on different scale information, thus it cannot generate satisfactory result by every layer.
}
\label{fig:cnnvis}
%\vspace{-14pt}
%\label{fig:pipline}
\end{figure}


==> Figs/fig_vit.tex <==
\newcommand\vitfigurewidth{0.32}

\begin{figure}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/c1.png}
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/r1.png}
\includegraphics[width=\vitfigurewidth\linewidth,height=\vitfigurewidth\linewidth]{image/figs_vits/s1.png}

\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/c2.png}
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/r2.png}
\includegraphics[width=\vitfigurewidth\linewidth,height=\vitfigurewidth\linewidth]{image/figs_vits/s2.png}

\vspace{-5pt}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{VIT}
\end{minipage}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\vspace{-7pt}
\caption{Style transfer results using model trained by VIT-based loss. 
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:vit}
\end{figure}


==> Figs/teaset.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/fig1.pdf}
\caption{Our style transfer results compared with state-of-the-art methods.}
\label{fig:position}
\vspace{-10pt}
\end{figure*}


==> Tables/tab_supp_progressive.tex <==
\begin{table}%[!h]
\small
\setlength\tabcolsep{2.5pt}
\centering
\begin{tabular}{c|c|c}
\toprule
&Single-layer &Ours (multi-layer)  \\
\midrule
$\contentloss$ $\downarrow$ & 1.94& \textbf{1.91} \\
$\styleloss$ $\downarrow$ & 2.38 & \textbf{1.47}  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Quantitative evaluation of progressive generation.}
\label{tab:loss1}
\end{table}


==> Tables/tab_timing_comparison.tex <==
\begin{table*}%[!h]
%\small
%\setlength\tabcolsep{2.5pt}
\centering
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{c|ccccccccccc}
\toprule
Resolution & Ours & StyleFormer&IEST&AdaAttN&ArtFlow & MCC &MAST&  AAMS & SANet&Avatar&AdaIN \\
\midrule
256 $\times$ 256&0.116 & 0.013&0.065& 0.104 & 0.142 & 0.013 &0.030& 2.074 & 0.015&0.260&0.007 \\
\midrule
512 $\times$ 512 & 0.661& 0.026& 0.092& 0.213 & 0.418 & 0.015  & 0.096&2.173 &0.019& 0.470&0.008 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\caption{Average inference time (in seconds) of different methods at two output resolutions.}
\label{tab:time}
\vspace{-7pt}
\end{table*}


==> Tables/tab_user_study.tex <==
% \begin{table}
%     \centering
%     \begin{subtable}[t]{\linewidth}
%         \begin{tabular}{c|ccccc}
%             \toprule
%             &ArtFlow&MCC&DFP& AAMS& AdaIN \\
%             \midrule
%             % Num. & 783&820&827&809&734 \\
%             votes(\%) &25.7&25.5&22.6&18.2& 23.5\\
%             % Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
%             \bottomrule
%         \end{tabular}
%         \caption{Overall}
%     \end{subtable}
%     \begin{subtable}[t]{\linewidth}
%     \begin{tabular}{c|ccccc}
%         % \begin{tabular}{m{0.6cm}<{\centering}|m{0.8cm}<{\centering}m{0.5cm}<{\centering}m{0.4cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
%             \toprule
%             &ArtFlow&MCC&DFP& AAMS& AdaIN \\
%             \midrule
%             % Num. & 783&820&827&809&734 \\
%             votes(\%) &28.3&20.6&9.2&19.4& 31.7\\
%             % Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
%             \bottomrule
%         \end{tabular}
%         \caption{Content}
%     \end{subtable}
%     \begin{subtable}[t]{\linewidth}
%         % \begin{tabular}{m{0.7cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
%         \begin{tabular}{c|ccccc}
%             \toprule
%             &ArtFlow&MCC&DFP& AAMS& AdaIN \\
%             \midrule
%             % Num. & 783&820&827&809&734 \\
%             votes(\%) &16.7&27.8&28.2&14.8& 13.5\\
%             % Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
%             \bottomrule
%         \end{tabular}
%         \caption{Style}
%     \end{subtable}
%     \caption{User study results.}
%     \label{tab:user_study}
% \end{table}
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{l|ccccc}
    \toprule
    &AdaAttN&ArtFlow & MCC  & AAMS & AdaIN \\
    \midrule
    Overall & 44.8\%&25.7\% & 25.5\%  & 18.2\% & 23.5\% \\
    \midrule
    Content & 45.7\%&28.3\% & 20.6\% & 19.4\%&  31.7\% \\
    \midrule
    Style & 23.6\%&16.7\% & 27.8\% & 14.8\% & 13.5\% \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\caption{User study results. Each number represents the percentage of votes that the corresponding method is preferred to ours, using the criteria of overall quality, preservation of content and style, respectively.}
\label{tab:user_study}
\vspace{-10pt}
\end{table}

